RayFlow: Instance-Aware Diffusion Acceleration via Adaptive Flow Trajectories

Diffusion models have achieved remarkable success across various domains. However, their slow generation speed remains a critical challenge. Existing acceleration methods, while aiming to reduce steps, often compromise sample quality, controllability, or introduce training complexities. Therefore, we propose RayFlow, a novel diffusion framework that addresses these limitations. Unlike previous methods, RayFlow guides each sample along a unique path towards an instance-specific target distribution. This method minimizes sampling steps while preserving generation diversity and stability. Furthermore, we introduce Time Sampler, an importance sampling technique to enhance training efficiency by focusing on crucial timesteps. Extensive experiments demonstrate RayFlow's superiority in generating high-quality images with improved speed, control, and training efficiency compared to existing acceleration techniques.

==> sec/RelatedWork.tex <==
\section{Related Work}
Diffusion models have demonstrated significant advancements across various applications, including data synthesis, density estimation, text-to-image generation, and more. Despite their strong performance, a major limitation of diffusion models is the requirement for a large number of sampling steps to generate realistic samples. This has led to the development of methods to distill pre-trained diffusion models into more efficient models.

\subsection{Trajectory Distillation}
Trajectory distillation methods train a student model to mimic the generation process of diffusion models with fewer steps. Direct distillation and progressive distillation are two variants that predict less noisy data from noisy inputs. Consistency-based methods minimize the self-consistency metric. These approaches, however, typically require true data samples for training \cite{huang2022masked, kim2021distilling}.

\subsection{Distributional Matching}
Distributional matching focuses on aligning the student's generation distribution with that of a teacher diffusion model. Adversarial training methods, which require real data for distilling diffusion models, fall under this category. These methods have shown promising results but often involve complex training procedures and high computational costs \cite{meng2023distillation, nichol2022glide}.

\subsection{Score Implicit Matching (SIM)}
A recent advancement in diffusion distillation is the Score Implicit Matching (SIM) approach, introduced by \cite{luo2024one}. SIM distills pre-trained diffusion models into single-step generator models while maintaining almost the same sample generation ability as the original model. The method is data-free, requiring no training samples for distillation. It leverages a wide class of score-based divergences between a diffusion model and a generator, efficiently computing gradients using the score-gradient theorem.

\subsection{KL and Fisher Divergence Minimization}
Previous works have explored diffusion distillation through the lens of probability divergence minimization. \cite{luo2024one} and \cite{yin2024kl} studied algorithms that minimize the KL divergence between teacher and one-step student models. \cite{zhou2024fisher} explored distilling with Fisher divergences, resulting in impressive empirical performances. However, these methods are built upon specific divergences, potentially restricting their distillation performances.

\subsection{Empirical Performance and Robustness}
SIM with a specially-designed Pseudo-Huber distance function shows faster convergence and stronger robustness to hyper-parameters than L2 distance, making it substantially stronger than previous approaches. The empirical results of SIM on CIFAR10 image generation and text-to-image generation demonstrate its effectiveness and robustness, marking a new direction for one-step text-to-image generation and motivating further studies in other domains such as video generation \cite{song2023distillation}.
